Context-Aware Transformer Pre-Training for Answer Sentence Selection

Answer Sentence Selection (AS2) is a core component for building an accurate Question Answering pipeline. AS2 models rank a set of candidate sentences based on how likely they answer a given question. The state of the art in AS2 exploits pre-trained transformers by transferring them on large annotated datasets, while using local contextual information around the candidate sentence. In this paper, we propose three pre-training objectives designed to mimic the downstream fine-tuning task of contextual AS2. This allows for specializing LMs when fine-tuning for contextual AS2. Our experiments on three public and two large-scale industrial datasets show that our pre-training approaches (applied to RoBERTa and ELECTRA) can improve baseline contextual AS2 accuracy by up to 8% on some datasets.

==> AS2_only_mlm_table.tex <==
\begin{table*}[t!]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lccccccccccccccc}
    \toprule
    \multirow{2}{*}{\textbf{Model+ Data Sampling}} & \multicolumn{3}{c}{\textbf{ASNQ}} & &\multicolumn{3}{c}{\textbf{WikiQA}} & & \multicolumn{3}{c}{\textbf{TREC-QA}} & & \multicolumn{3}{c}{\textbf{WQA}} \\
    \cmidrule{2-4} \cmidrule{6-8} \cmidrule{10-12} \cmidrule{14-16}
                           & \textbf{P@1}    & \textbf{MAP}    & \textbf{MRR}   & &\textbf{ P@1}     & \textbf{MAP}     & \textbf{MRR}   & & \textbf{P@1}   & \textbf{MAP}     & \textbf{MRR}  & & \textbf{P@1}    & \textbf{MAP}    & \textbf{MRR}    \\
    \midrule
    
    RoBERTa-Base                                             & 61.8 {\small (0.2)} & 66.9 {\small (0.1)} & 73.1 {\small (0.1)}       & & 78.3 {\small (2.8)} & 85.8 {\small (1.3)} & 87.2 {\small (1.3)}     & & 90.0 {\small (1.9)} & 89.7 {\small (0.7)} & 94.4 {\small (1.1)}      & &  \multicolumn{3}{c}{Baseline}  \\

    \midrule

    + SSP Data (\textbf{MLM-only})   & 63.4 {\small (0.4)} & 67.1 {\small (0.2)} & 73.8 {\small (0.2)}       & & 76.7 {\small (0.9)} & 84.5 {\small (0.7)} & 85.8 {\small (0.7)}     & & 87.4 {\small (1.3)} & 88.8 {\small (0.6)} & 93.1 {\small (1.0)}      & & -0.6\%   & -0.2\%    & -0.3\% \\
    + SSP                            & \bfunder{64.1} {\small (0.3)} & \bfunder{68.1} {\small (0.2)} & \bfunder{74.5} {\small (0.3)}      & & \bfunder{82.9} {\small (0.7)} & \bfunder{88.7} {\small (0.3)} & \bfunder{89.9} {\small (0.4)}          & & \textbf{88.5} {\small (1.2)}  & \textbf{89.3} {\small (0.7)} & \textbf{93.6} {\small (0.6)}                               & & \bfunder{+0.2}\% & \bfunder{+0.6\%} & \bfunder{+0.3}\% \\

    \midrule

    + SP Data (\textbf{MLM-only})    & 62.8 {\small (0.3)} & 67.2 {\small (0.2)} & 73.7 {\small (0.2)}       & & 76.8 {\small (1.6)} & 84.7 {\small (0.8)} & 86.2 {\small (0.7)}     & & 88.8 {\small (1.3)} & 89.8 {\small (0.3)} & 93.7 {\small (0.9)}      & & -1.0\%   & -0.4\%    & -0.6\% \\
    + SP               & \bfunder{64.1} {\small (0.2)} & \bfunder{68.3} {\small (0.1)} & \bfunder{74.5} {\small (0.2)}        & & \bfunder{81.0} {\small (0.8)} & \bfunder{87.7} {\small (0.3)} & \bfunder{88.9} {\small (0.4)}    & & \textbf{90.9} {\small (2.6)} & \textbf{90.1} {\small (0.8)} & \textbf{94.7} {\small (1.3)}                       & & \bfunder{+0.4\%} & \bfunder{+0.7\%}  & \bfunder{+0.5\%} \\

    \midrule

    + PSD Data (\textbf{MLM-only})   & \bfunder{64.1} {\small (0.5)} & 67.3 {\small (0.2)} & 73.7 {\small (0.2)}       & & 79.1 {\small (1.6)} & 85.6 {\small (1.4)} & 87.1 {\small (1.2)}     & & 87.1 {\small (2.8)} & 89.6 {\small (1.0)} & 92.7 {\small (1.3)}      & & -1.3\%   & -0.3\%    & -0.6\% \\
    + PSD                            & 62.6 {\small (0.4)} & \bfunder{67.7} {\small (0.2)} & 73.7 {\small (0.3)}              & & \textbf{80.5} {\small (1.6)} & \textbf{86.4} {\small (1.1)} & \textbf{88.0} {\small (1.0)}                                        & & \bfunder{90.3} {\small (1.3)} & \textbf{90.3} {\small (0.5)} & \bfunder{95.1} {\small (0.7)}              & & \bfunder{+0.4\%}  & \bfunder{+0.7\%} & \bfunder{+0.5\%} \\

    \bottomrule

    \end{tabular}
    }
    \caption{Results (with std. dev. across 5 runs in parentheses) of our pretrained transformer models when fine-tuned on AS2 datasets with MLM-only pre-training. SSP, SP and PSD refer to our pretraining objectives. Results on WQA are relative to RoBERTa baseline. We highlight in bold and underline results like in Table \ref{tab:results_as2}.}
    \label{tab:results_as2_only_mlm}
\end{table*}


==> AS2_only_mlm_table_small.tex <==
\begin{table}[t!]
    \centering
    \resizebox{0.85\linewidth}{!}{
    \begin{tabular}{lcccc}
    \toprule
    \textbf{Model+Data Sampling} & \textbf{ASNQ} & \textbf{WikiQA} & \textbf{TREC-QA} & \textbf{WQA} \\

    \midrule

    RoBERTa-Base                                   & 61.8                & 78.3               & 90.0  & Baseline \\

    \midrule

    + SSP Data (\textbf{MLM-only})        & 63.4               & 76.7               & 87.4            & -0.6\% \\
    + SSP                & \bfunder{64.1}     & \bfunder{82.9}     & \textbf{88.5}   & \bfunder{+0.2}\% \\

    \midrule

    + SP Data (\textbf{MLM-only})        & 62.8               & 76.8              & 88.8             & -1.0\% \\
    + SP                 & \bfunder{64.1}     & \bfunder{81.0}     & \textbf{90.9}   & \bfunder{+0.4}\% \\

    \midrule

    + PSD Data (\textbf{MLM-only})        & \bfunder{64.1}     & 79.1               & 87.1             & -1.3\% \\
    + PSD                & 62.6               & \bfunder{80.5}     & \bfunder{90.3}   & \bfunder{+0.4}\% \\

    \bottomrule

    \end{tabular}
    }
    \caption{P@1 of our pretrained models using SSP, SP and PSD objectives in addition to only MLM. We highlight in bold and underline results like in Table \ref{tab:results_as2}.}
    \label{tab:results_as2_only_mlm_small}
\end{table}


==> AS2_table.tex <==
\begin{table*}[t!]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lccccccccccccccc}
    \toprule
    \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{ASNQ}} & &\multicolumn{3}{c}{\textbf{WikiQA}} & & \multicolumn{3}{c}{\textbf{TREC-QA}} & & \multicolumn{3}{c}{\textbf{WQA}} \\
    \cmidrule{2-4} \cmidrule{6-8} \cmidrule{10-12} \cmidrule{14-16}
                           & \textbf{P@1}    & \textbf{MAP}    & \textbf{MRR}   & &\textbf{ P@1}     & \textbf{MAP}     & \textbf{MRR}   & & \textbf{P@1}   & \textbf{MAP}     & \textbf{MRR}  & & \textbf{P@1}    & \textbf{MAP}    & \textbf{MRR}    \\
    \midrule
    
    RoBERTa-Base     & 61.8 {\small (0.2)} & 66.9 {\small (0.1)} & 73.1 {\small (0.1)}                                      & & 78.3 {\small (2.8)} & 85.8 {\small (1.3)} & 87.2 {\small (1.3)}                                        & & 90.0 {\small (1.9)}  & 89.7 {\small (0.7)} & 94.4 {\small (1.1)}                               & & \multicolumn{3}{c}{Baseline}  \\
    {\small (\textbf{Ours})} RoBERTa + SSP       & \bfunder{64.1} {\small (0.3)} & \underline{68.1} {\small (0.2)} & \bfunder{74.5} {\small (0.3)}      & & \bfunder{82.9} {\small (0.7)} & \bfunder{88.7} {\small (0.3)} & \bfunder{89.9} {\small (0.4)}          & & 88.5 {\small (1.2)}  & 89.3 {\small (0.7)} & 93.6 {\small (0.6)}                               & & +0.2\% & \underline{+0.6\%} & +0.3\% \\
    {\small (\textbf{Ours})} RoBERTa + SP      & \bfunder{64.1} {\small (0.2)} & \bfunder{68.3} {\small (0.1)} & \bfunder{74.5} {\small (0.2)}        & & \underline{81.0} {\small (0.8)} & \underline{87.7} {\small (0.3)} & \underline{88.9} {\small (0.4)}    & & \textbf{90.9} {\small (2.6)} & 90.1 {\small (0.8)} & 94.7 {\small (1.3)}                       & & \underline{+0.4\%} & \underline{+0.7\%}  & \underline{+0.5\%} \\
    {\small (\textbf{Ours})} RoBERTa + PSD      & 62.6 {\small (0.4)} & \underline{67.7} {\small (0.2)} & \underline{73.7} {\small (0.3)}              & & 80.5 {\small (1.6)} & 86.4 {\small (1.1)} & 88.0 {\small (1.0)}                                        & & 90.3 {\small (1.3)} & \textbf{90.3} {\small (0.5)} & \textbf{95.1} {\small (0.7)}              & & \underline{+0.4\%}  & \underline{+0.7\%} & \underline{+0.5\%} \\
    
    {\small (\textbf{Ours})} RoBERTa + All      & \underline{63.9} {\small (0.4)} & \underline{68.0} {\small (0.1)} & \underline{74.1} {\small (0.2)}              & & \underline{82.5} {\small (0.9)} & \underline{88.2} {\small (0.4)} & \underline{89.5} {\small (0.4)}                                        & & 87.9 {\small (1.2)} & \textbf{89.3} {\small (0.7)} & \textbf{93.4} {\small (0.6)}              & & \bfunder{+0.5\%}  & \bfunder{+0.8\%} & \bfunder{+0.6\%} \\
    TANDA RoBERTa         & -     & -     & -     & & 83.0 {\small (1.3)}    & 88.5 {\small (0.8)}   & 89.9 {\small (0.8)}  & & 89.7 {\small (0.0)}    & 90.1 {\small (0.6)} & 94.1 {\small (0.4)}  & & +0.5\%   & +0.5\%    & +0.5\% \\
    
    \midrule

    ELECTRA-Base    & 62.4 {\small (0.4)} & 67.5 {\small (0.2)} & 73.6 {\small (0.2)}                                      & & 77.1 {\small (4.0)} & 85.0 {\small (2.6)} & 86.5 {\small (2.7)}                                        & & 90.3 {\small (1.7)} & 89.9 {\small (0.4)} & 94.0 {\small (0.9)}                                & & +1.0\%  & +1.2\% & +0.9\% \\
    {\small (\textbf{Ours})} ELECTRA + SSP       & \bfunder{65.3} {\small (0.3)} & \bfunder{69.7} {\small (0.2)} & \bfunder{75.7} {\small (0.2)}        & & \bfunder{82.5} {\small (2.0)} & \bfunder{88.6} {\small (1.4)} & \bfunder{90.0} {\small (1.4)}          & & 88.5 {\small (1.9)} & 89.6 {\small (0.7)} & 93.5 {\small (0.9)}                                & & \underline{+1.4\%} & \underline{+1.5\%} & \underline{+1.3\%} \\
    {\small (\textbf{Ours})} ELECTRA + SP      & \underline{65.0} {\small (0.2)} & \underline{69.0} {\small (0.1)} & \underline{75.1} {\small (0.1)}  & & \underline{81.8} {\small (2.3)} & \underline{88.1} {\small (1.5)} & \underline{89.5} {\small (1.5)}    & & 91.2 {\small (1.5)} & 90.3 {\small (0.7)} & 94.6 {\small (0.7)}     & & \underline{+1.4\%} & \underline{+1.5\%} & \underline{+1.3\%} \\
    {\small (\textbf{Ours})} ELECTRA + PSD      & \bfunder{65.3} {\small (0.4)} & \underline{68.9} {\small (0.3)} & \underline{75.1} {\small (0.3)}    & & 78.6 {\small (0.7)} & 85.6 {\small (0.7)} & 87.3 {\small (0.6)}                                        & & 85.9 {\small (2.2)} & 87.9 {\small (1.1)} & 92.2 {\small (1.1)}                                & & \bfunder{+1.6\%}  & \bfunder{+1.6\%} & \underline{+1.3\%} \\
    {\small (\textbf{Ours})} ELECTRA + All      & \underline{65.0} {\small (0.3)} & \underline{69.3} {\small (0.2)} & \underline{75.2} {\small (0.2)}    & & 80.8 {\small (1.9)} & 87.3 {\small (1.2)} & \underline{88.7} {\small (1.1)}                                        & & \bfunder{92.6} {\small (1.8)} & \textbf{90.4} {\small (0.4)} & \textbf{95.5} {\small (1.0)}                                & & \underline{+1.5\%}  & \bfunder{+1.6\%} & \bfunder{+1.4\%} \\
    TANDA ELECTRA         & -     & -     & -     & & 85.6 {\small (1.1)}    & 90.2 {\small (0.8)}   & 91.4 {\small (0.7)}  & & 92.6 {\small (1.5)}    & 91.6 {\small (0.7)} & 95.5 {\small (0.7)}  & & +1.9\%   & +1.6\%   & +1.5\% \\
    \bottomrule

    \end{tabular}
    }
    \caption{Results (with std. dev. across 5 runs in parentheses) of our pretrained transformers when fine-tuned on AS2 datasets. SSP, SP, PSD denote our pretraining objectives, and `All' denotes using SSP+SP+PSD together. TANDA uses \textbf{additional labeled data} as an intermediate transfer step. We underline statistically significant improvements over the baseline (T-test at a 95\% confidence level). Results on WQA are relative to the RoBERTa baseline.}
    \label{tab:results_as2}
\end{table*}

==> [ACL 2023] - Context-Aware Transformer Pre-Training for AS2/AS2_only_mlm_table.tex <==
\begin{table*}[t!]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lccccccccccccccc}
    \toprule
    \multirow{2}{*}{\textbf{Model+ Data Sampling}} & \multicolumn{3}{c}{\textbf{ASNQ}} & &\multicolumn{3}{c}{\textbf{WikiQA}} & & \multicolumn{3}{c}{\textbf{TREC-QA}} & & \multicolumn{3}{c}{\textbf{WQA}} \\
    \cmidrule{2-4} \cmidrule{6-8} \cmidrule{10-12} \cmidrule{14-16}
                           & \textbf{P@1}    & \textbf{MAP}    & \textbf{MRR}   & &\textbf{ P@1}     & \textbf{MAP}     & \textbf{MRR}   & & \textbf{P@1}   & \textbf{MAP}     & \textbf{MRR}  & & \textbf{P@1}    & \textbf{MAP}    & \textbf{MRR}    \\
    \midrule
    
    RoBERTa-Base                                             & 61.8 {\small (0.2)} & 66.9 {\small (0.1)} & 73.1 {\small (0.1)}       & & 78.3 {\small (2.8)} & 85.8 {\small (1.3)} & 87.2 {\small (1.3)}     & & 90.0 {\small (1.9)} & 89.7 {\small (0.7)} & 94.4 {\small (1.1)}      & &  \multicolumn{3}{c}{Baseline}  \\

    \midrule

    + SSP Data (\textbf{MLM-only})   & 63.4 {\small (0.4)} & 67.1 {\small (0.2)} & 73.8 {\small (0.2)}       & & 76.7 {\small (0.9)} & 84.5 {\small (0.7)} & 85.8 {\small (0.7)}     & & 87.4 {\small (1.3)} & 88.8 {\small (0.6)} & 93.1 {\small (1.0)}      & & -0.6\%   & -0.2\%    & -0.3\% \\
    + SSP                            & \bfunder{64.1} {\small (0.3)} & \bfunder{68.1} {\small (0.2)} & \bfunder{74.5} {\small (0.3)}      & & \bfunder{82.9} {\small (0.7)} & \bfunder{88.7} {\small (0.3)} & \bfunder{89.9} {\small (0.4)}          & & \textbf{88.5} {\small (1.2)}  & \textbf{89.3} {\small (0.7)} & \textbf{93.6} {\small (0.6)}                               & & \bfunder{+0.2}\% & \bfunder{+0.6\%} & \bfunder{+0.3}\% \\

    \midrule

    + SP Data (\textbf{MLM-only})    & 62.8 {\small (0.3)} & 67.2 {\small (0.2)} & 73.7 {\small (0.2)}       & & 76.8 {\small (1.6)} & 84.7 {\small (0.8)} & 86.2 {\small (0.7)}     & & 88.8 {\small (1.3)} & 89.8 {\small (0.3)} & 93.7 {\small (0.9)}      & & -1.0\%   & -0.4\%    & -0.6\% \\
    + SP               & \bfunder{64.1} {\small (0.2)} & \bfunder{68.3} {\small (0.1)} & \bfunder{74.5} {\small (0.2)}        & & \bfunder{81.0} {\small (0.8)} & \bfunder{87.7} {\small (0.3)} & \bfunder{88.9} {\small (0.4)}    & & \textbf{90.9} {\small (2.6)} & \textbf{90.1} {\small (0.8)} & \textbf{94.7} {\small (1.3)}                       & & \bfunder{+0.4\%} & \bfunder{+0.7\%}  & \bfunder{+0.5\%} \\

    \midrule

    + PSD Data (\textbf{MLM-only})   & \bfunder{64.1} {\small (0.5)} & 67.3 {\small (0.2)} & 73.7 {\small (0.2)}       & & 79.1 {\small (1.6)} & 85.6 {\small (1.4)} & 87.1 {\small (1.2)}     & & 87.1 {\small (2.8)} & 89.6 {\small (1.0)} & 92.7 {\small (1.3)}      & & -1.3\%   & -0.3\%    & -0.6\% \\
    + PSD                            & 62.6 {\small (0.4)} & \bfunder{67.7} {\small (0.2)} & 73.7 {\small (0.3)}              & & \textbf{80.5} {\small (1.6)} & \textbf{86.4} {\small (1.1)} & \textbf{88.0} {\small (1.0)}                                        & & \bfunder{90.3} {\small (1.3)} & \textbf{90.3} {\small (0.5)} & \bfunder{95.1} {\small (0.7)}              & & \bfunder{+0.4\%}  & \bfunder{+0.7\%} & \bfunder{+0.5\%} \\

    \bottomrule

    \end{tabular}
    }
    \caption{Results (with std. dev. across 5 runs in parentheses) of our pretrained transformer models when fine-tuned on AS2 datasets with MLM-only pre-training. SSP, SP and PSD refer to our pretraining objectives. Results on WQA are relative to RoBERTa baseline. We highlight in bold and underline results like in Table \ref{tab:results_as2}.}
    \label{tab:results_as2_only_mlm}
\end{table*}


==> [ACL 2023] - Context-Aware Transformer Pre-Training for AS2/AS2_only_mlm_table_small.tex <==
\begin{table}[t!]
    \centering
    \resizebox{0.85\linewidth}{!}{
    \begin{tabular}{lcccc}
    \toprule
    \textbf{Model+Data Sampling} & \textbf{ASNQ} & \textbf{WikiQA} & \textbf{TREC-QA} & \textbf{WQA} \\

    \midrule

    RoBERTa-Base                                   & 61.8                & 78.3               & 90.0  & Baseline \\

    \midrule

    + SSP Data (\textbf{MLM-only})        & 63.4               & 76.7               & 87.4            & -0.6\% \\
    + SSP                & \bfunder{64.1}     & \bfunder{82.9}     & \textbf{88.5}   & \bfunder{+0.2}\% \\

    \midrule

    + SP Data (\textbf{MLM-only})        & 62.8               & 76.8              & 88.8             & -1.0\% \\
    + SP                 & \bfunder{64.1}     & \bfunder{81.0}     & \textbf{90.9}   & \bfunder{+0.4}\% \\

    \midrule

    + PSD Data (\textbf{MLM-only})        & \bfunder{64.1}     & 79.1               & 87.1             & -1.3\% \\
    + PSD                & 62.6               & \bfunder{80.5}     & \bfunder{90.3}   & \bfunder{+0.4}\% \\

    \bottomrule

    \end{tabular}
    }
    \caption{P@1 of our pretrained models using SSP, SP and PSD objectives in addition to only MLM. We highlight in bold and underline results like in Table \ref{tab:results_as2}.}
    \label{tab:results_as2_only_mlm_small}
\end{table}


==> [ACL 2023] - Context-Aware Transformer Pre-Training for AS2/AS2_stats.tex <==
\begin{table}[t]
\centering
\small
\resizebox{\linewidth}{!}{
    
\begin{tabular}{lccccccccc}
    \toprule
    \multirow{2}{*}{\textbf{Dataset}} & \multicolumn{2}{c}{\textbf{Train}} & & \multicolumn{2}{c}{\textbf{Dev}} & & \multicolumn{2}{c}{\textbf{Test}} \\ \cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-9} & \textbf{\#Q} & \textbf{\#QA} & & \textbf{\#Q} & \textbf{\#QA} & & \textbf{\#Q} & \textbf{\#QA} \\

    \midrule
    ASNQ                    & 57242	& 20377568                                      && 1336 & 463914                                    && 1336 & 466148 \\
    \midrule
    WikiQA                    & 2118	& 20360                                      && 122 & 1126                                    && 237 & 2341 \\
    \midrule
    \multirow{2}{*}{IQAD}   & \multirow{2}{*}{221334} & \multirow{2}{*}{3894129}    && \multirow{2}{*}{2434} &
    \multirow{2}{*}{43369}   && 2252 & 38587 \\
                            & &                                                     && &                                                && 2088 & 33498 \\
    \midrule
    NewsAS2                  & 71561	& 1840533                                       && 2102 & 51844                                     && 2083 & 51472 \\
\bottomrule
\end{tabular}
}
\vspace{0.3em}
\caption{Number or unique questions and question-answer pairs in the fine-tuning datasets. IQAD Bench 1 and Bench 2 sizes are mentioned in the Test set column corresponding to IQAD.}
\label{tab:datasets_stats}
\end{table}


==> [ACL 2023] - Context-Aware Transformer Pre-Training for AS2/AS2_table.tex <==
\begin{table*}[t!]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lccccccccccccccc}
    \toprule
    \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{ASNQ}} & &\multicolumn{3}{c}{\textbf{WikiQA}} & & \multicolumn{3}{c}{\textbf{TREC-QA}} & & \multicolumn{3}{c}{\textbf{WQA}} \\
    \cmidrule{2-4} \cmidrule{6-8} \cmidrule{10-12} \cmidrule{14-16}
                           & \textbf{P@1}    & \textbf{MAP}    & \textbf{MRR}   & &\textbf{ P@1}     & \textbf{MAP}     & \textbf{MRR}   & & \textbf{P@1}   & \textbf{MAP}     & \textbf{MRR}  & & \textbf{P@1}    & \textbf{MAP}    & \textbf{MRR}    \\
    \midrule
    
    RoBERTa-Base     & 61.8 {\small (0.2)} & 66.9 {\small (0.1)} & 73.1 {\small (0.1)}                                      & & 78.3 {\small (2.8)} & 85.8 {\small (1.3)} & 87.2 {\small (1.3)}                                        & & 90.0 {\small (1.9)}  & 89.7 {\small (0.7)} & 94.4 {\small (1.1)}                               & & \multicolumn{3}{c}{Baseline}  \\
    {\small (\textbf{Ours})} RoBERTa + SSP       & \bfunder{64.1} {\small (0.3)} & \underline{68.1} {\small (0.2)} & \bfunder{74.5} {\small (0.3)}      & & \bfunder{82.9} {\small (0.7)} & \bfunder{88.7} {\small (0.3)} & \bfunder{89.9} {\small (0.4)}          & & 88.5 {\small (1.2)}  & 89.3 {\small (0.7)} & 93.6 {\small (0.6)}                               & & +0.2\% & \underline{+0.6\%} & +0.3\% \\
    {\small (\textbf{Ours})} RoBERTa + SP      & \bfunder{64.1} {\small (0.2)} & \bfunder{68.3} {\small (0.1)} & \bfunder{74.5} {\small (0.2)}        & & \underline{81.0} {\small (0.8)} & \underline{87.7} {\small (0.3)} & \underline{88.9} {\small (0.4)}    & & \textbf{90.9} {\small (2.6)} & 90.1 {\small (0.8)} & 94.7 {\small (1.3)}                       & & \underline{+0.4\%} & \underline{+0.7\%}  & \underline{+0.5\%} \\
    {\small (\textbf{Ours})} RoBERTa + PSD      & 62.6 {\small (0.4)} & \underline{67.7} {\small (0.2)} & \underline{73.7} {\small (0.3)}              & & 80.5 {\small (1.6)} & 86.4 {\small (1.1)} & 88.0 {\small (1.0)}                                        & & 90.3 {\small (1.3)} & \textbf{90.3} {\small (0.5)} & \textbf{95.1} {\small (0.7)}              & & \underline{+0.4\%}  & \underline{+0.7\%} & \underline{+0.5\%} \\
    
    {\small (\textbf{Ours})} RoBERTa + All      & \underline{63.9} {\small (0.4)} & \underline{68.0} {\small (0.1)} & \underline{74.1} {\small (0.2)}              & & \underline{82.5} {\small (0.9)} & \underline{88.2} {\small (0.4)} & \underline{89.5} {\small (0.4)}                                        & & 87.9 {\small (1.2)} & \textbf{89.3} {\small (0.7)} & \textbf{93.4} {\small (0.6)}              & & \bfunder{+0.5\%}  & \bfunder{+0.8\%} & \bfunder{+0.6\%} \\
    TANDA RoBERTa         & -     & -     & -     & & 83.0 {\small (1.3)}    & 88.5 {\small (0.8)}   & 89.9 {\small (0.8)}  & & 89.7 {\small (0.0)}    & 90.1 {\small (0.6)} & 94.1 {\small (0.4)}  & & +0.5\%   & +0.5\%    & +0.5\% \\
    
    \midrule

    ELECTRA-Base    & 62.4 {\small (0.4)} & 67.5 {\small (0.2)} & 73.6 {\small (0.2)}                                      & & 77.1 {\small (4.0)} & 85.0 {\small (2.6)} & 86.5 {\small (2.7)}                                        & & 90.3 {\small (1.7)} & 89.9 {\small (0.4)} & 94.0 {\small (0.9)}                                & & +1.0\%  & +1.2\% & +0.9\% \\
    {\small (\textbf{Ours})} ELECTRA + SSP       & \bfunder{65.3} {\small (0.3)} & \bfunder{69.7} {\small (0.2)} & \bfunder{75.7} {\small (0.2)}        & & \bfunder{82.5} {\small (2.0)} & \bfunder{88.6} {\small (1.4)} & \bfunder{90.0} {\small (1.4)}          & & 88.5 {\small (1.9)} & 89.6 {\small (0.7)} & 93.5 {\small (0.9)}                                & & \underline{+1.4\%} & \underline{+1.5\%} & \underline{+1.3\%} \\
    {\small (\textbf{Ours})} ELECTRA + SP      & \underline{65.0} {\small (0.2)} & \underline{69.0} {\small (0.1)} & \underline{75.1} {\small (0.1)}  & & \underline{81.8} {\small (2.3)} & \underline{88.1} {\small (1.5)} & \underline{89.5} {\small (1.5)}    & & 91.2 {\small (1.5)} & 90.3 {\small (0.7)} & 94.6 {\small (0.7)}     & & \underline{+1.4\%} & \underline{+1.5\%} & \underline{+1.3\%} \\
    {\small (\textbf{Ours})} ELECTRA + PSD      & \bfunder{65.3} {\small (0.4)} & \underline{68.9} {\small (0.3)} & \underline{75.1} {\small (0.3)}    & & 78.6 {\small (0.7)} & 85.6 {\small (0.7)} & 87.3 {\small (0.6)}                                        & & 85.9 {\small (2.2)} & 87.9 {\small (1.1)} & 92.2 {\small (1.1)}                                & & \bfunder{+1.6\%}  & \bfunder{+1.6\%} & \underline{+1.3\%} \\
    {\small (\textbf{Ours})} ELECTRA + All      & \underline{65.0} {\small (0.3)} & \underline{69.3} {\small (0.2)} & \underline{75.2} {\small (0.2)}    & & 80.8 {\small (1.9)} & 87.3 {\small (1.2)} & \underline{88.7} {\small (1.1)}                                        & & \bfunder{92.6} {\small (1.8)} & \textbf{90.4} {\small (0.4)} & \textbf{95.5} {\small (1.0)}                                & & \underline{+1.5\%}  & \bfunder{+1.6\%} & \bfunder{+1.4\%} \\
    TANDA ELECTRA         & -     & -     & -     & & 85.6 {\small (1.1)}    & 90.2 {\small (0.8)}   & 91.4 {\small (0.7)}  & & 92.6 {\small (1.5)}    & 91.6 {\small (0.7)} & 95.5 {\small (0.7)}  & & +1.9\%   & +1.6\%   & +1.5\% \\
    \bottomrule

    \end{tabular}
    }
    \caption{Results (with std. dev. across 5 runs in parentheses) of our pretrained transformers when fine-tuned on AS2 datasets. SSP, SP, PSD denote our pretraining objectives, and `All' denotes using SSP+SP+PSD together. TANDA uses \textbf{additional labeled data} as an intermediate transfer step. We underline statistically significant improvements over the baseline (T-test at a 95\% confidence level). Results on WQA are relative to the RoBERTa baseline.}
    \label{tab:results_as2}
\end{table*}

==> [ACL 2023] - Context-Aware Transformer Pre-Training for AS2/pretraining_table.tex <==
\iffalse
\begin{table}[t!]
    \centering
    \resizebox{0.8\linewidth}{!}{
    \begin{tabular}{lccc}
    \toprule
    \textbf{Model+ Pre-training Objective} & \textbf{Accuracy} & \textbf{F1} \\
    \midrule
    \textbf{SP (Span in Paragraph)} &&\\
    RoBERTa-Base      & 91.8   & 83.1 \\
    ELECTRA-Base      & 90.4   & 79.9 \\
    \midrule
    \textbf{SSP (Spans in Same Paragraph)} &&\\
    RoBERTa-Base + SSP     & 91.3   & 83.3 \\
    ELECTRA-Base + SSP     & 89.9   & 80.1 \\
    \midrule
    \textbf{PSD (Paragraphs in Same Document)} &&\\
    RoBERTa-Base + PSD     & 83.5   & 61.4 \\
    ELECTRA-Base + PSD     & 82.3   & 57.1 \\
    \midrule
    BERT~\cite{devlin-etal-2019-bert} (NSP) & 96.9 & 97.1\\
    ALBERT~\cite{lan2020albert} (SOP) & 93.7 & 94.7\\
    \bottomrule
    \end{tabular}
    }
    \caption{Comparison of accuracy and F1-score of pre-training objectives on the pre-training validation set.}
    \label{tab:results_pretraining}
\end{table}
\fi
%we may compress (and fix) the table as follows

\begin{table}[t!]
    \centering
    \resizebox{0.7\linewidth}{!}{
    \begin{tabular}{lccc}
    \toprule
    \textbf{Model + Pre-training Objective} & \textbf{Accuracy} & \textbf{F1} \\
    \midrule
    RoBERTa-Base + \textbf{SSP}      & 91.8   & 83.1 \\
    ELECTRA-Base + \textbf{SSP}      & 90.4   & 79.9 \\
    \midrule
    RoBERTa-Base + \textbf{SP}     & 91.3   & 83.3 \\
    ELECTRA-Base + \textbf{SP}     & 89.9   & 80.1 \\
    \midrule
    RoBERTa-Base + \textbf{PSD}     & 83.5   & 61.4 \\
    ELECTRA-Base + \textbf{PSD}     & 82.3   & 57.1 \\
    \midrule
    BERT~\cite{devlin-etal-2019-bert} (NSP) & 96.9 & 97.1\\
    ALBERT~\cite{lan2020albert} (SOP) & 93.7 & 94.7\\
    \bottomrule
    \end{tabular}
    }
    \caption{Comparison of accuracy and F1-score of pre-training objectives on the pre-training validation set.}
    \label{tab:results_pretraining}
\end{table}


==> [ACL 2023] - Context-Aware Transformer Pre-Training for AS2/table.tex <==
\begin{table*}[t]
\centering
\resizebox{\linewidth}{!}{
    
\begin{tabular}{lccccccccccccccc}
    \toprule
    \multirow{2}[3]{*}{\textbf{Model}} & \multirow{2}[3]{*}{\textbf{\shortstack{Context}}} & \multicolumn{2}{c}{\textbf{ASNQ}} & & \multicolumn{2}{c}{\textbf{WikiQA}} & & \multicolumn{2}{c}{\textbf{NewsAS2}} & & \multicolumn{2}{c}{\textbf{IQAD Bench 1}} & & \multicolumn{2}{c}{\textbf{IQAD Bench 2}} \\
    
    \cmidrule{3-4} \cmidrule{6-7} \cmidrule{9-10} \cmidrule{12-13} \cmidrule{15-16} &  & \textbf{MAP} & \textbf{P@1} & & \textbf{MAP} & \textbf{P@1} & & \textbf{MAP} & \textbf{P@1} & & \textbf{MAP} &\textbf{P@1} & & \textbf{MAP} &\textbf{P@1} \\

\midrule

ELECTRA-Base   & {\xmark}                               & 69.3 (0.0) & 65.0 (0.2)               & & 85.7 (0.9) & 78.5 (1.6)                 & & 81.3 (0.2) & 75.6 (0.2)                 & & \multicolumn{2}{c}{Baseline}        & & \multicolumn{2}{c}{Baseline} \\
ELECTRA-Base~$\clubsuit$ & {\cmark}                     & 72.3 (0.6) & 68.1 (0.8)               & & 83.1 (1.3) & 73.8 (2.1)                 & & 82.0 (0.4) & 76.0 (0.5)                 & & -0.6\% & -1.0\%                     & & -0.4\% & -0.9\% \\

\midrule

\textbf{(Ours)} ELECTRA-Base + SSP (SDC) & {\cmark}     & \bund{74.7} (0.5) & \und{69.6} (0.3)  & & \bund{88.7} (0.1) & \bund{82.9} (0.2)   & & \und{82.7} (0.2) & 77.0 (0.4)           & & \bund{+1.2\%} & \textbf{+0.6\%}     & & \bund{+0.9\%} & \bund{+1.4\%} \\
\textbf{(Ours)} ELECTRA-Base + SSP (DPC) & {\cmark}     & \und{74.4} (0.2)  & \bund{70.5} (0.2) & & \und{88.0} (0.6) & \und{81.3} (0.6)     & & 82.7 (0.5) & \bund{77.3} (0.7)          & & +0.4\% & -0.6\%                     & & +0.4\% & +0.1\% \\
\textbf{(Ours)} ELECTRA-Base + SSP (DSLC) & {\cmark}    & \und{74.3} (0.3)  & \und{70.0} (0.8)  & & \und{87.0} (0.9) & \und{79.7} (1.4)     & & \textbf{82.8} (0.4) & \bund{77.3} (0.5) & & \und{+1.0\%} & +0.6\%               & & \und{+0.2\%} & 0.0\%  \\
\textbf{(Ours)} ELECTRA-Base + SSP (All) & {\cmark}     & \und{73.8} (0.4)  & 68.8 (0.4)        & & \und{87.5} (0.5) & \und{81.5} (0.7)     & & \und{82.7} (0.2) & \und{77.2} (0.3)     & & +0.1\% & -0.4\%                     & & +0.1\% & -0.1\% \\

\midrule
\midrule

RoBERTa-Base & {\xmark}                                 & 68.2 (0.5) & 63.5 (0.5)               & & 85.1 (1.9) & 77.2 (3.1)                 & & 81.7 (0.1) & 76.2 (0.2)                 & & +0.6\% & +0.1\%                     & & +0.7\% & +1.3\% \\
RoBERTa-Base~$\clubsuit$  & {\cmark}                    & 71.6 (0.6) & 67.6 (0.6)               & & 84.4 (1.5) & 77.0 (2.1)                 & & 82.4 (0.2) & 76.6 (0.7)                 & & +0.4\% & 0.0\%                      & & +1.1\% & +1.7\% \\

\midrule

\textbf{(Ours)} RoBERTa-Base + SSP (SDC) & {\cmark}     & \und{73.1} (0.5) & 68.7 (0.8)         & & \und{87.8} (0.6) & \und{81.8} (0.9)     & & \und{82.8} (0.1) & 76.9 (0.2)           & & \bund{+1.7\%} & \bund{+3.0\%}       & & +1.0\% & +1.7\% \\
\textbf{(Ours)} RoBERTa-Base + SSP (DPC) & {\cmark}     & \bund{73.2} (0.4) & \bund{69.2} (0.5) & & \bund{89.9} (0.2) & \bund{85.2} (0.4)   & & 82.3 (0.1) & 76.0 (0.1)                 & & +0.4\% & +1.2\%                     & & +1.2\% & \bund{+2.7\%} \\
\textbf{(Ours)} RoBERTa-Base + SSP (DSLC) & {\cmark}    & \und{72.9} (0.4) & \und{69.0} (0.3)   & & \und{87.8} (0.9) & \und{81.6} (1.3)     & & 82.6 (0.2) & 77.0 (0.2)                 & & +0.6\% & +1.5\%                     & & +1.0\% & +1.4\% \\
\textbf{(Ours)} RoBERTa-Base + SSP (All) & {\cmark}     & 72.9 (0.6) & 68.2 (0.8)               & & \und{88.2} (0.9) & \und{82.4} (1.7)     & & \bund{83.0} (0.2) & \textbf{77.3} (0.5) & & \und{+1.2\%} & \und{+2.4\%}         & & \textbf{+1.4\%} & +2.2\% \\

    \bottomrule
\end{tabular}
}

\vspace{0.3em}
\caption{Results (std. dev. in parenthesis) on AS2. Models with $\clubsuit$ are from \cite{Lauriola2021}. {\cmark} and {\xmark} denote whether local contextual information was used in fine-tuning. SDC, DPC and DSLC indicate the pre-training variants of the SSP task that we propose.
%``All'' refers to the combination of our three pre-training objectives.
Best results are in bold while we underline statistically significant improvements over the two contextual baselines ($\clubsuit$) using a Student \textit{t}-test with $95\%$ of confidence level.}
\vspace{0.3em}
\label{tab:results_as2}
\end{table*}







% Table backup
\iffalse

\begin{table*}[ht]
\centering
\resizebox{\linewidth}{!}{
    
\begin{tabular}{lcccccccccccccccc}
    \toprule
    \multirow{2}[3]{*}{\textbf{Model}} & \multirow{2}[3]{*}{\textbf{\shortstack{Context\\ used}}} & \multicolumn{3}{c}{\textbf{ASNQ}} & & \multicolumn{3}{c}{\textbf{NewsAS2}} & & \multicolumn{3}{c}{\textbf{IQAD Bench 1}} & & \multicolumn{3}{c}{\textbf{IQAD Bench 2}} \\ \cmidrule{3-5} \cmidrule{7-9} \cmidrule{11-13} \cmidrule{15-17} &  & \textbf{MAP} & \textbf{MRR} & \textbf{P@1} & & \textbf{MAP} & \textbf{MRR} & \textbf{P@1} & & \textbf{MAP} & \textbf{MRR} & \textbf{P@1} & & \textbf{MAP} & \textbf{MRR} & \textbf{P@1} \\

\midrule

ELECTRA-Base   & {\xmark}                               & 69.3 (0.0) & 75.1 (0.1) & 65.0 (0.2)                      & & 81.3 (0.2) & 84.2 (0.1) & 75.6 (0.2)                            & & \multicolumn{3}{c}{Baseline}                        & & \multicolumn{3}{c}{Baseline} \\
ELECTRA-Base~$\clubsuit$ & {\cmark}                     & 72.3 (0.6) & 77.9 (0.8) & 68.1 (0.8)                      & & 82.0 (0.4) & 84.6 (0.2) & 76.0 (0.5)                            & & -0.6\% & -0.6\% & -1.0\%                            & & -0.4\% & -0.4\% & -0.9\% \\

\midrule

\textbf{(Ours)} ELECTRA-Base + SSP (SDC) & {\cmark}     & \bund{74.7} (0.5) & \bund{79.5} (0.3) & \und{69.6} (0.3)  & & \und{82.7} (0.2) & \und{85.3} (0.3) & 77.0 (0.4)                & & \bund{+1.2\%} & \textbf{+0.6\%} & \textbf{+0.6\%}   & & \bund{+0.9\%} & \bund{+0.9\%} & \bund{+1.4\%} \\
\textbf{(Ours)} ELECTRA-Base + SSP (DPC) & {\cmark}     & \und{74.4} (0.2) & \bund{79.5} (0.2) & \bund{70.5} (0.2)  & & 82.7 (0.5) & \bund{85.6} (0.4) & \bund{77.3} (0.7)              & & +0.4\% & -0.3\% & -0.6\%                            & & +0.4\% & +0.2\% & +0.1\% \\
\textbf{(Ours)} ELECTRA-Base + SSP (DSLC) & {\cmark}    & \und{74.3} (0.3) & \und{79.4} (0.5) & \und{70.0} (0.8)    & & \textbf{82.8} (0.4) & \und{85.5} (0.4) & \bund{77.3} (0.5)      & & \und{+1.0\%} & +0.5\% & +0.6\%                      & & \und{+0.2\%} & \und{+0.2\%} & 0.0\%  \\
\textbf{(Ours)} ELECTRA-Base + SSP (All) & {\cmark}     & \und{73.8} (0.4) & 78.7 (0.3) & 68.8 (0.4)                & & \und{82.7} (0.2) & \und{85.4} (0.2) & \und{77.2} (0.3)          & & +0.1\% & -0.1\% & -0.4\%                            & & +0.1\% & +0.1\% & -0.1\% \\

\midrule
\midrule

RoBERTa-Base & {\xmark}                                 & 68.2 (0.5) & 74.2 (0.3) & 63.5 (0.5)                      & & 81.7 (0.1) & 84.4 (0.0) & 76.2 (0.2)                            & & +0.6\% & +0.5\% & +0.1\%                            & & +0.7\% & +0.9\% & +1.3\% \\
% RoBERTa-Base \cite{Lauriola2021} Local                & 73.2	     & 75.2       & 65.3 \\
% RoBERTa-Base \cite{Lauriola2021} Global               & 69.8       & 72.2	      & 62.2 \\
RoBERTa-Base~$\clubsuit$  & {\cmark}                     & 71.6 (0.6) & 77.3 (0.5) &	67.6 (0.6)                      & & 82.4 (0.2) & 85.1 (0.4) & 76.6 (0.7)                            & & +0.4\% & +0.4\% & 0.0\%                             & & +1.1\% & +0.9\% & +1.7\% \\

\midrule

\textbf{(Ours)} RoBERTa-Base + SSP (SDC) & {\cmark}     & \und{73.1} (0.5) & 78.4 (0.6) & 68.7 (0.8)                & & \und{82.8} (0.1) & 85.4 (0.2) & 76.9 (0.2)                      & & \bund{+1.7\%} & \bund{+1.8\%} & \bund{+3.0\%}       & & +1.0\% & +0.9\% & +1.7\% \\
\textbf{(Ours)} RoBERTa-Base + SSP (DPC) & {\cmark}     & \bund{73.2} (0.4) & \bund{78.5} (0.3) & \bund{69.2} (0.5) & & 82.3 (0.1) & 84.9 (0.1) & 76.0 (0.1)                            & & +0.4\% & +0.6\% & +1.2\%                            & & +1.2\% & \textbf{+1.5\%} & \bund{+2.7\%} \\
\textbf{(Ours)} RoBERTa-Base + SSP (DSLC) & {\cmark}    & \und{72.9} (0.4) & \und{78.4} (0.2) & \und{69.0} (0.3)    & & 82.6 (0.2) & 85.3 (0.1) & 77.0 (0.2)                            & & +0.6\% & +0.9\% & +1.5\%                            & & +1.0\% & +0.9\% & +1.4\% \\
\textbf{(Ours)} RoBERTa-Base + SSP (All) & {\cmark}     & 72.9 (0.6) & 77.9 (0.6) & 68.2 (0.8)                      & & \bund{83.0} (0.2) & \textbf{85.6} (0.4) & \textbf{77.3} (0.5)   & & \und{+1.2\%} & \und{+1.5\%} & \und{+2.4\%}                      & & \textbf{+1.4\%} & +1.3\% & +2.2\% \\

    \bottomrule
\end{tabular}
}
\vspace{0.3em}
\caption{Results (std. dev. in parenthesis) on AS2. Models with $\clubsuit$ are from \cite{Lauriola2021}. {\cmark} and {\xmark} denote whether local contextual information was used in fine-tuning. SDC, DPC and DSLC indicate the pre-training variants of the SSP task that we propose.
%``All'' refers to the combination of our three pre-training objectives.
Best results are in bold while we underline statistically significant improvements over the two contextual baselines ($\clubsuit$) using a Student \textit{t}-test with $95\%$ of confidence level.}
\vspace{0.3em}
\label{tab:results_as2}
\end{table*}



\fi

==> pretraining_table.tex <==
\iffalse
\begin{table}[t!]
    \centering
    \resizebox{0.8\linewidth}{!}{
    \begin{tabular}{lccc}
    \toprule
    \textbf{Model+ Pre-training Objective} & \textbf{Accuracy} & \textbf{F1} \\
    \midrule
    \textbf{SP (Span in Paragraph)} &&\\
    RoBERTa-Base      & 91.8   & 83.1 \\
    ELECTRA-Base      & 90.4   & 79.9 \\
    \midrule
    \textbf{SSP (Spans in Same Paragraph)} &&\\
    RoBERTa-Base + SSP     & 91.3   & 83.3 \\
    ELECTRA-Base + SSP     & 89.9   & 80.1 \\
    \midrule
    \textbf{PSD (Paragraphs in Same Document)} &&\\
    RoBERTa-Base + PSD     & 83.5   & 61.4 \\
    ELECTRA-Base + PSD     & 82.3   & 57.1 \\
    \midrule
    BERT~\cite{devlin-etal-2019-bert} (NSP) & 96.9 & 97.1\\
    ALBERT~\cite{lan2020albert} (SOP) & 93.7 & 94.7\\
    \bottomrule
    \end{tabular}
    }
    \caption{Comparison of accuracy and F1-score of pre-training objectives on the pre-training validation set.}
    \label{tab:results_pretraining}
\end{table}
\fi
%we may compress (and fix) the table as follows

\begin{table}[t!]
    \centering
    \resizebox{0.7\linewidth}{!}{
    \begin{tabular}{lccc}
    \toprule
    \textbf{Model + Pre-training Objective} & \textbf{Accuracy} & \textbf{F1} \\
    \midrule
    RoBERTa-Base + \textbf{SSP}      & 91.8   & 83.1 \\
    ELECTRA-Base + \textbf{SSP}      & 90.4   & 79.9 \\
    \midrule
    RoBERTa-Base + \textbf{SP}     & 91.3   & 83.3 \\
    ELECTRA-Base + \textbf{SP}     & 89.9   & 80.1 \\
    \midrule
    RoBERTa-Base + \textbf{PSD}     & 83.5   & 61.4 \\
    ELECTRA-Base + \textbf{PSD}     & 82.3   & 57.1 \\
    \midrule
    BERT~\cite{devlin-etal-2019-bert} (NSP) & 96.9 & 97.1\\
    ALBERT~\cite{lan2020albert} (SOP) & 93.7 & 94.7\\
    \bottomrule
    \end{tabular}
    }
    \caption{Comparison of accuracy and F1-score of pre-training objectives on the pre-training validation set.}
    \label{tab:results_pretraining}
\end{table}

